MDMMT: Multidomain Multimodal Transformer for Video Retrieval

We present a new state-of-the-art on the text to video retrieval task on MSRVTT and LSMDC benchmarks where our model outperforms all previous solutions by a large margin. Moreover, state-of-the-art results are achieved with a single model on two datasets without finetuning. This multidomain generalisation is achieved by a proper combination of different video caption datasets. We show that training on different datasets can improve test results of each other. Additionally we check intersection between many popular datasets and found that MSRVTT has a significant overlap between the test and the train parts, and the same situation is observed for ActivityNet.

==> tables/activitynet_arch_epe_gpu.tex <==
MALVYMTSK & L4H4 & 150 & 1 & 8.09 \textpm 0.14 & 23.45 \textpm 0.59 & 34.59 \textpm 0.51 & 166.29 \textpm 2.69 & 23.00 \textpm 0.00 \\
MALVYMTSK & L4H4 & 150 & 8 & 10.35 \textpm 0.34 & 28.93 \textpm 0.27 & 41.64 \textpm 0.43 & 139.54 \textpm 0.73 & 15.67 \textpm 0.47 \\
MALVYMTSK & L4H4 & 32 & 1 & 5.58 \textpm 0.22 & 18.01 \textpm 0.16 & 27.56 \textpm 0.15 & 206.95 \textpm 2.23 & 34.00 \textpm 0.00 \\
MALVYMTSK & L4H4 & 32 & 8 & 8.35 \textpm 0.33 & 24.65 \textpm 0.11 & 35.86 \textpm 0.05 & 161.20 \textpm 2.26 & 21.00 \textpm 0.00 \\
MALVYMTSK & L6H8 & 150 & 1 & 8.09 \textpm 0.54 & 23.98 \textpm 0.57 & 34.78 \textpm 0.49 & 164.81 \textpm 3.60 & 23.00 \textpm 0.00 \\
MALVYMTSK & L6H8 & 150 & 8 & 10.77 \textpm 0.20 & 29.30 \textpm 0.27 & 41.57 \textpm 0.39 & 138.34 \textpm 1.39 & 15.67 \textpm 0.47 \\
MALVYMTSK & L6H8 & 32 & 1 & 5.64 \textpm 0.03 & 17.46 \textpm 0.39 & 26.98 \textpm 0.23 & 209.03 \textpm 5.22 & 34.67 \textpm 1.25 \\
MALVYMTSK & L6H8 & 32 & 8 & 8.65 \textpm 0.01 & 24.93 \textpm 0.12 & 36.04 \textpm 0.18 & 159.12 \textpm 2.93 & 20.67 \textpm 0.47 \\
MALVYMT & L4H4 & 150 & 1 & 8.44 \textpm 0.19 & 24.35 \textpm 0.25 & 35.91 \textpm 0.28 & 153.78 \textpm 2.25 & 20.33 \textpm 0.47 \\
MALVYMT & L4H4 & 150 & 8 & 10.53 \textpm 0.14 & 29.58 \textpm 0.43 & 42.51 \textpm 0.29 & 135.14 \textpm 3.37 & 15.00 \textpm 0.82 \\
MALVYMT & L4H4 & 32 & 1 & 5.94 \textpm 0.09 & 19.03 \textpm 0.30 & 28.79 \textpm 0.23 & 188.46 \textpm 2.56 & 31.33 \textpm 0.47 \\
MALVYMT & L4H4 & 32 & 8 & 9.19 \textpm 0.07 & 25.92 \textpm 0.42 & 37.64 \textpm 0.22 & 144.92 \textpm 1.82 & 19.00 \textpm 0.00 \\
MALVYMT & L6H8 & 150 & 1 & 8.42 \textpm 0.23 & 24.49 \textpm 0.03 & 36.21 \textpm 0.39 & 152.42 \textpm 2.79 & 21.00 \textpm 0.00 \\
MALVYMT & L6H8 & 150 & 8 & 11.10 \textpm 0.19 & 30.29 \textpm 0.23 & 42.40 \textpm 0.39 & 134.60 \textpm 1.78 & 15.33 \textpm 0.47 \\
MALVYMT & L6H8 & 32 & 1 & 6.21 \textpm 0.10 & 18.91 \textpm 0.08 & 28.82 \textpm 0.12 & 187.49 \textpm 1.12 & 33.00 \textpm 0.82 \\
MALVYMT & L6H8 & 32 & 8 & 9.31 \textpm 0.15 & 25.90 \textpm 0.29 & 37.51 \textpm 0.15 & 145.81 \textpm 1.01 & 19.00 \textpm 0.00 \\
MALV & L4H4 & 150 & 1 & 8.34 \textpm 0.21 & 24.92 \textpm 0.82 & 36.68 \textpm 0.68 & 150.85 \textpm 2.45 & 19.67 \textpm 0.47 \\
MALV & L4H4 & 150 & 8 & 10.15 \textpm 0.38 & 29.33 \textpm 0.23 & 42.50 \textpm 0.66 & 140.70 \textpm 1.69 & 15.33 \textpm 0.47 \\
MALV & L4H4 & 32 & 1 & 6.12 \textpm 0.31 & 19.36 \textpm 0.10 & 29.00 \textpm 0.41 & 182.65 \textpm 3.31 & 30.33 \textpm 1.25 \\
MALV & L4H4 & 32 & 8 & 8.36 \textpm 0.14 & 25.74 \textpm 0.33 & 37.87 \textpm 0.23 & 147.88 \textpm 1.90 & 18.67 \textpm 0.47 \\
MALV & L6H8 & 150 & 1 & 8.26 \textpm 0.12 & 24.61 \textpm 0.24 & 36.04 \textpm 0.47 & 151.42 \textpm 0.87 & 20.67 \textpm 0.47 \\
MALV & L6H8 & 150 & 8 & 10.51 \textpm 0.27 & 30.01 \textpm 0.29 & 42.78 \textpm 0.45 & 141.81 \textpm 0.96 & 14.67 \textpm 0.47 \\
MALV & L6H8 & 32 & 1 & 6.26 \textpm 0.07 & 19.92 \textpm 0.29 & 29.49 \textpm 0.83 & 178.32 \textpm 5.98 & 29.67 \textpm 1.25 \\
MALV & L6H8 & 32 & 8 & 8.96 \textpm 0.18 & 26.63 \textpm 0.09 & 38.59 \textpm 0.28 & 145.21 \textpm 2.24 & 18.33 \textpm 0.47 \\
M & L4H4 & 150 & 1 & 3.86 \textpm 0.08 & 12.66 \textpm 0.34 & 19.69 \textpm 0.62 & 349.79 \textpm 5.77 & 65.33 \textpm 0.94 \\
M & L4H4 & 150 & 8 & 4.13 \textpm 0.18 & 13.32 \textpm 0.05 & 20.39 \textpm 0.27 & 405.63 \textpm 5.99 & 71.00 \textpm 2.16 \\
M & L4H4 & 32 & 1 & 4.19 \textpm 0.21 & 13.00 \textpm 0.38 & 20.15 \textpm 0.13 & 299.62 \textpm 3.21 & 59.67 \textpm 0.94 \\
M & L4H4 & 32 & 8 & 4.55 \textpm 0.22 & 14.29 \textpm 0.21 & 21.72 \textpm 0.36 & 324.23 \textpm 6.56 & 55.67 \textpm 1.25 \\
M & L6H8 & 150 & 1 & 4.40 \textpm 0.21 & 13.01 \textpm 0.19 & 19.87 \textpm 0.28 & 346.71 \textpm 4.59 & 66.00 \textpm 0.82 \\
M & L6H8 & 150 & 8 & 4.38 \textpm 0.25 & 13.32 \textpm 0.11 & 20.53 \textpm 0.15 & 399.88 \textpm 10.05 & 72.33 \textpm 0.94 \\
M & L6H8 & 32 & 1 & 3.71 \textpm 0.03 & 12.96 \textpm 0.07 & 20.02 \textpm 0.10 & 306.12 \textpm 3.62 & 61.67 \textpm 1.25 \\
M & L6H8 & 32 & 8 & 4.47 \textpm 0.18 & 14.55 \textpm 0.48 & 22.07 \textpm 0.35 & 325.39 \textpm 3.04 & 57.00 \textpm 1.63 \\


==> tables/k700_arch_epe_gpu.tex <==
MALVYMTSK & L4H4 & 150 & 1 & 4.40 \textpm 0.23 & 12.93 \textpm 0.50 & 19.28 \textpm 0.68 & 610.88 \textpm 13.54 & 78.67 \textpm 3.30 \\
MALVYMTSK & L4H4 & 150 & 8 & 8.99 \textpm 0.24 & 24.10 \textpm 0.32 & 33.15 \textpm 0.26 & 370.51 \textpm 5.59 & 31.33 \textpm 0.47 \\
MALVYMTSK & L4H4 & 32 & 1 & 1.79 \textpm 0.06 & 6.40 \textpm 0.16 & 10.46 \textpm 0.19 & 981.91 \textpm 11.65 & 178.33 \textpm 2.49 \\
MALVYMTSK & L4H4 & 32 & 8 & 4.71 \textpm 0.31 & 14.35 \textpm 0.29 & 21.18 \textpm 0.30 & 571.85 \textpm 19.47 & 67.00 \textpm 0.82 \\
MALVYMTSK & L6H8 & 150 & 1 & 4.02 \textpm 0.03 & 12.57 \textpm 0.08 & 18.92 \textpm 0.15 & 589.42 \textpm 7.47 & 79.00 \textpm 0.82 \\
MALVYMTSK & L6H8 & 150 & 8 & 9.65 \textpm 0.18 & 24.51 \textpm 0.17 & 33.57 \textpm 0.20 & 366.97 \textpm 8.08 & 30.33 \textpm 0.47 \\
MALVYMTSK & L6H8 & 32 & 1 & 1.94 \textpm 0.23 & 6.76 \textpm 0.49 & 10.74 \textpm 0.60 & 945.53 \textpm 32.39 & 174.67 \textpm 7.41 \\
MALVYMTSK & L6H8 & 32 & 8 & 4.72 \textpm 0.11 & 14.28 \textpm 0.05 & 21.04 \textpm 0.16 & 562.06 \textpm 5.33 & 68.00 \textpm 0.82 \\
MALVYMT & L4H4 & 150 & 1 & 1.92 \textpm 0.08 & 6.16 \textpm 0.15 & 9.28 \textpm 0.02 & 2618.55 \textpm 32.25 & 381.33 \textpm 7.36 \\
MALVYMT & L4H4 & 150 & 8 & 2.87 \textpm 0.07 & 8.28 \textpm 0.16 & 11.94 \textpm 0.13 & 2700.02 \textpm 90.84 & 324.00 \textpm 8.83 \\
MALVYMT & L4H4 & 32 & 1 & 1.09 \textpm 0.09 & 4.10 \textpm 0.19 & 6.77 \textpm 0.35 & 2699.29 \textpm 128.43 & 457.67 \textpm 21.06 \\
MALVYMT & L4H4 & 32 & 8 & 2.34 \textpm 0.07 & 7.06 \textpm 0.12 & 10.55 \textpm 0.13 & 2418.42 \textpm 13.80 & 316.33 \textpm 3.68 \\
MALVYMT & L6H8 & 150 & 1 & 1.85 \textpm 0.03 & 5.67 \textpm 0.08 & 8.78 \textpm 0.20 & 2634.02 \textpm 119.48 & 389.33 \textpm 15.80 \\
MALVYMT & L6H8 & 150 & 8 & 2.77 \textpm 0.20 & 8.15 \textpm 0.48 & 11.98 \textpm 0.50 & 2680.06 \textpm 57.62 & 328.00 \textpm 20.70 \\
MALVYMT & L6H8 & 32 & 1 & 1.10 \textpm 0.09 & 3.87 \textpm 0.18 & 6.42 \textpm 0.25 & 2673.13 \textpm 64.56 & 462.67 \textpm 14.61 \\
MALVYMT & L6H8 & 32 & 8 & 2.24 \textpm 0.15 & 7.05 \textpm 0.24 & 10.46 \textpm 0.29 & 2356.26 \textpm 56.19 & 318.33 \textpm 6.94 \\
MALV & L4H4 & 150 & 1 & 1.78 \textpm 0.03 & 5.57 \textpm 0.18 & 8.39 \textpm 0.24 & 2976.56 \textpm 68.91 & 459.33 \textpm 3.30 \\
MALV & L4H4 & 150 & 8 & 2.57 \textpm 0.06 & 7.66 \textpm 0.22 & 11.07 \textpm 0.23 & 3114.70 \textpm 40.78 & 424.33 \textpm 8.38 \\
MALV & L4H4 & 32 & 1 & 1.13 \textpm 0.11 & 3.67 \textpm 0.21 & 5.99 \textpm 0.18 & 2818.48 \textpm 95.78 & 514.33 \textpm 21.36 \\
MALV & L4H4 & 32 & 8 & 2.17 \textpm 0.15 & 6.49 \textpm 0.21 & 9.68 \textpm 0.26 & 2746.30 \textpm 69.58 & 377.67 \textpm 18.12 \\
MALV & L6H8 & 150 & 1 & 1.59 \textpm 0.26 & 5.19 \textpm 0.61 & 8.18 \textpm 0.67 & 2923.27 \textpm 28.50 & 486.00 \textpm 15.77 \\
MALV & L6H8 & 150 & 8 & 2.55 \textpm 0.12 & 7.67 \textpm 0.08 & 11.07 \textpm 0.08 & 3016.51 \textpm 55.01 & 415.67 \textpm 12.04 \\
MALV & L6H8 & 32 & 1 & 0.93 \textpm 0.09 & 3.43 \textpm 0.34 & 5.70 \textpm 0.43 & 2822.05 \textpm 68.07 & 533.33 \textpm 20.07 \\
MALV & L6H8 & 32 & 8 & 2.23 \textpm 0.14 & 6.32 \textpm 0.08 & 9.66 \textpm 0.07 & 2732.99 \textpm 83.74 & 386.00 \textpm 18.18 \\
M & L4H4 & 150 & 1 & 1.08 \textpm 0.15 & 3.41 \textpm 0.22 & 5.39 \textpm 0.20 & 3903.01 \textpm 60.69 & 793.00 \textpm 25.35 \\
M & L4H4 & 150 & 8 & 1.50 \textpm 0.15 & 4.37 \textpm 0.22 & 6.61 \textpm 0.14 & 4157.17 \textpm 87.39 & 851.33 \textpm 25.77 \\
M & L4H4 & 32 & 1 & 0.83 \textpm 0.05 & 3.02 \textpm 0.08 & 4.97 \textpm 0.14 & 3244.10 \textpm 33.18 & 654.33 \textpm 9.84 \\
M & L4H4 & 32 & 8 & 1.28 \textpm 0.04 & 4.21 \textpm 0.13 & 6.65 \textpm 0.33 & 3312.30 \textpm 52.13 & 610.67 \textpm 15.08 \\
M & L6H8 & 150 & 1 & 0.99 \textpm 0.11 & 3.30 \textpm 0.16 & 5.20 \textpm 0.14 & 3959.77 \textpm 114.51 & 851.33 \textpm 39.91 \\
M & L6H8 & 150 & 8 & 1.32 \textpm 0.15 & 4.08 \textpm 0.13 & 6.33 \textpm 0.09 & 4139.14 \textpm 6.43 & 852.00 \textpm 36.18 \\
M & L6H8 & 32 & 1 & 0.90 \textpm 0.05 & 3.08 \textpm 0.03 & 5.00 \textpm 0.06 & 3266.25 \textpm 44.97 & 683.00 \textpm 11.22 \\
M & L6H8 & 32 & 8 & 1.22 \textpm 0.03 & 4.09 \textpm 0.11 & 6.46 \textpm 0.21 & 3433.43 \textpm 33.30 & 644.67 \textpm 13.70 \\


==> tables/msrvtt_arch_epe_gpu.tex <==

MALVYMTSK & L4H4 & 150 & 1 & 22.30 \textpm 1.15 & 51.23 \textpm 1.16 & 63.80 \textpm 0.29 & 27.22 \textpm 0.64 & 5.33 \textpm 0.47 \\
MALVYMTSK & L4H4 & 150 & 8 & 25.33 \textpm 0.52 & 53.97 \textpm 0.12 & 65.73 \textpm 0.57 & 30.20 \textpm 0.95 & 4.67 \textpm 0.47 \\
MALVYMTSK & L4H4 & 32 & 1 & 17.50 \textpm 0.96 & 44.40 \textpm 1.24 & 58.87 \textpm 0.33 & 29.95 \textpm 0.42 & 7.00 \textpm 0.00 \\
MALVYMTSK & L4H4 & 32 & 8 & 24.57 \textpm 0.31 & 53.23 \textpm 0.26 & 66.73 \textpm 0.41 & 25.24 \textpm 0.43 & 5.00 \textpm 0.00 \\
MALVYMTSK & L6H8 & 150 & 1 & 22.70 \textpm 0.43 & 49.93 \textpm 0.76 & 64.30 \textpm 0.65 & 27.68 \textpm 0.46 & 5.67 \textpm 0.47 \\
MALVYMTSK & L6H8 & 150 & 8 & 25.27 \textpm 0.47 & 54.90 \textpm 0.22 & 67.27 \textpm 0.60 & 29.73 \textpm 1.04 & 4.00 \textpm 0.00 \\
MALVYMTSK & L6H8 & 32 & 1 & 17.90 \textpm 0.65 & 44.47 \textpm 0.62 & 58.97 \textpm 0.76 & 30.03 \textpm 0.58 & 7.00 \textpm 0.00 \\
MALVYMTSK & L6H8 & 32 & 8 & 24.20 \textpm 0.79 & 53.10 \textpm 0.29 & 66.57 \textpm 0.83 & 25.27 \textpm 0.93 & 5.00 \textpm 0.00 \\
MALVYMT & L4H4 & 150 & 1 & 24.03 \textpm 0.12 & 51.93 \textpm 0.66 & 65.67 \textpm 0.24 & 25.91 \textpm 0.05 & 5.00 \textpm 0.00 \\
MALVYMT & L4H4 & 150 & 8 & 25.50 \textpm 0.64 & 54.23 \textpm 0.29 & 65.60 \textpm 0.67 & 32.10 \textpm 1.48 & 4.00 \textpm 0.00 \\
MALVYMT & L4H4 & 32 & 1 & 19.67 \textpm 0.74 & 46.13 \textpm 0.76 & 60.77 \textpm 0.21 & 27.58 \textpm 0.60 & 6.33 \textpm 0.47 \\
MALVYMT & L4H4 & 32 & 8 & 26.10 \textpm 0.59 & 53.80 \textpm 0.57 & 66.27 \textpm 0.42 & 25.47 \textpm 0.38 & 4.33 \textpm 0.47 \\
MALVYMT & L6H8 & 150 & 1 & 23.73 \textpm 0.74 & 51.80 \textpm 0.94 & 65.03 \textpm 0.69 & 26.02 \textpm 0.72 & 5.00 \textpm 0.00 \\
MALVYMT & L6H8 & 150 & 8 & 26.70 \textpm 1.14 & 53.83 \textpm 0.96 & 66.57 \textpm 0.63 & 31.38 \textpm 0.83 & 4.67 \textpm 0.47 \\
MALVYMT & L6H8 & 32 & 1 & 19.70 \textpm 0.43 & 46.07 \textpm 0.12 & 60.40 \textpm 0.82 & 28.60 \textpm 0.72 & 6.00 \textpm 0.00 \\
MALVYMT & L6H8 & 32 & 8 & 24.70 \textpm 0.86 & 53.83 \textpm 0.76 & 66.60 \textpm 0.24 & 25.53 \textpm 0.89 & 4.67 \textpm 0.47 \\
MALV & L4H4 & 150 & 1 & 22.07 \textpm 0.45 & 50.03 \textpm 0.95 & 63.50 \textpm 0.49 & 28.47 \textpm 0.31 & 5.67 \textpm 0.47 \\
MALV & L4H4 & 150 & 8 & 23.00 \textpm 0.86 & 51.13 \textpm 0.19 & 63.87 \textpm 0.73 & 35.88 \textpm 1.01 & 5.00 \textpm 0.00 \\
MALV & L4H4 & 32 & 1 & 18.90 \textpm 0.41 & 46.83 \textpm 0.83 & 61.23 \textpm 0.68 & 28.01 \textpm 0.91 & 6.33 \textpm 0.47 \\
MALV & L4H4 & 32 & 8 & 24.43 \textpm 0.29 & 52.23 \textpm 0.54 & 64.97 \textpm 0.38 & 28.04 \textpm 0.49 & 5.00 \textpm 0.00 \\
MALV & L6H8 & 150 & 1 & 21.60 \textpm 0.14 & 50.33 \textpm 0.52 & 62.73 \textpm 0.45 & 28.28 \textpm 0.73 & 5.33 \textpm 0.47 \\
MALV & L6H8 & 150 & 8 & 23.00 \textpm 0.22 & 51.50 \textpm 0.86 & 63.70 \textpm 0.08 & 36.41 \textpm 0.96 & 5.00 \textpm 0.00 \\
MALV & L6H8 & 32 & 1 & 19.40 \textpm 0.59 & 47.43 \textpm 0.17 & 60.63 \textpm 0.62 & 28.02 \textpm 0.53 & 6.33 \textpm 0.47 \\
MALV & L6H8 & 32 & 8 & 23.10 \textpm 0.29 & 52.03 \textpm 0.83 & 64.40 \textpm 0.14 & 27.70 \textpm 0.88 & 5.00 \textpm 0.00 \\
M & L4H4 & 150 & 1 & 19.83 \textpm 0.53 & 48.63 \textpm 0.88 & 61.47 \textpm 0.39 & 37.08 \textpm 1.24 & 6.00 \textpm 0.00 \\
M & L4H4 & 150 & 8 & 19.13 \textpm 0.80 & 44.77 \textpm 0.50 & 56.57 \textpm 0.54 & 48.66 \textpm 3.54 & 7.33 \textpm 0.47 \\
M & L4H4 & 32 & 1 & 20.23 \textpm 0.39 & 48.13 \textpm 1.10 & 62.03 \textpm 0.88 & 29.65 \textpm 0.60 & 6.00 \textpm 0.00 \\
M & L4H4 & 32 & 8 & 21.60 \textpm 0.24 & 49.97 \textpm 0.33 & 61.70 \textpm 0.57 & 35.62 \textpm 0.68 & 5.33 \textpm 0.47 \\
M & L6H8 & 150 & 1 & 20.13 \textpm 0.50 & 47.13 \textpm 1.11 & 59.97 \textpm 1.03 & 36.09 \textpm 1.32 & 6.67 \textpm 0.47 \\
M & L6H8 & 150 & 8 & 20.57 \textpm 0.12 & 45.63 \textpm 0.49 & 56.27 \textpm 0.26 & 49.97 \textpm 1.06 & 7.00 \textpm 0.00 \\
M & L6H8 & 32 & 1 & 20.27 \textpm 0.87 & 47.13 \textpm 0.87 & 61.33 \textpm 0.24 & 28.86 \textpm 0.47 & 6.33 \textpm 0.47 \\
M & L6H8 & 32 & 8 & 21.67 \textpm 1.49 & 49.50 \textpm 0.49 & 61.47 \textpm 0.41 & 35.57 \textpm 0.75 & 5.67 \textpm 0.47 \\


==> tables/somethingV2_arch_epe_gpu.tex <==
MALVYMTSK & L4H4 & 150 & 1 & 2.89 \textpm 0.10 & 9.06 \textpm 0.20 & 14.04 \textpm 0.19 & 669.59 \textpm 6.00 & 138.00 \textpm 3.56 \\
MALVYMTSK & L4H4 & 150 & 8 & 4.33 \textpm 0.09 & 13.08 \textpm 0.16 & 19.40 \textpm 0.18 & 538.00 \textpm 2.82 & 84.33 \textpm 1.25 \\
MALVYMTSK & L4H4 & 32 & 1 & 1.52 \textpm 0.03 & 5.46 \textpm 0.06 & 8.84 \textpm 0.04 & 1004.85 \textpm 17.39 & 257.00 \textpm 6.53 \\
MALVYMTSK & L4H4 & 32 & 8 & 3.00 \textpm 0.08 & 9.58 \textpm 0.02 & 14.61 \textpm 0.17 & 665.41 \textpm 6.54 & 131.33 \textpm 1.25 \\
MALVYMTSK & L6H8 & 150 & 1 & 2.94 \textpm 0.11 & 9.35 \textpm 0.27 & 14.39 \textpm 0.28 & 658.90 \textpm 1.24 & 133.00 \textpm 1.41 \\
MALVYMTSK & L6H8 & 150 & 8 & 4.48 \textpm 0.08 & 13.70 \textpm 0.16 & 20.18 \textpm 0.07 & 516.16 \textpm 3.33 & 79.00 \textpm 0.82 \\
MALVYMTSK & L6H8 & 32 & 1 & 1.54 \textpm 0.04 & 5.43 \textpm 0.15 & 8.76 \textpm 0.17 & 1006.23 \textpm 6.79 & 254.33 \textpm 2.62 \\
MALVYMTSK & L6H8 & 32 & 8 & 3.15 \textpm 0.03 & 9.85 \textpm 0.17 & 15.21 \textpm 0.14 & 628.85 \textpm 4.83 & 123.67 \textpm 1.25 \\
MALVYMT & L4H4 & 150 & 1 & 0.34 \textpm 0.01 & 1.19 \textpm 0.04 & 1.98 \textpm 0.08 & 4190.94 \textpm 4.76 & 2076.33 \textpm 19.74 \\
MALVYMT & L4H4 & 150 & 8 & 0.40 \textpm 0.04 & 1.53 \textpm 0.06 & 2.48 \textpm 0.10 & 4043.82 \textpm 85.35 & 1842.00 \textpm 75.40 \\
MALVYMT & L4H4 & 32 & 1 & 0.28 \textpm 0.03 & 1.04 \textpm 0.06 & 1.81 \textpm 0.12 & 4521.38 \textpm 155.80 & 2412.67 \textpm 144.65 \\
MALVYMT & L4H4 & 32 & 8 & 0.42 \textpm 0.02 & 1.49 \textpm 0.02 & 2.51 \textpm 0.11 & 3997.62 \textpm 33.05 & 1862.67 \textpm 34.93 \\
MALVYMT & L6H8 & 150 & 1 & 0.30 \textpm 0.01 & 1.16 \textpm 0.04 & 2.00 \textpm 0.10 & 4297.87 \textpm 69.28 & 2142.33 \textpm 46.23 \\
MALVYMT & L6H8 & 150 & 8 & 0.35 \textpm 0.04 & 1.36 \textpm 0.11 & 2.22 \textpm 0.05 & 4114.54 \textpm 23.21 & 1934.67 \textpm 48.62 \\
MALVYMT & L6H8 & 32 & 1 & 0.27 \textpm 0.02 & 1.05 \textpm 0.05 & 1.82 \textpm 0.06 & 4533.69 \textpm 63.40 & 2415.67 \textpm 79.21 \\
MALVYMT & L6H8 & 32 & 8 & 0.41 \textpm 0.01 & 1.46 \textpm 0.03 & 2.40 \textpm 0.03 & 4020.52 \textpm 26.77 & 1863.67 \textpm 6.13 \\
MALV & L4H4 & 150 & 1 & 0.32 \textpm 0.04 & 1.06 \textpm 0.04 & 1.79 \textpm 0.09 & 4525.96 \textpm 62.38 & 2323.33 \textpm 42.12 \\
MALV & L4H4 & 150 & 8 & 0.36 \textpm 0.01 & 1.20 \textpm 0.03 & 2.00 \textpm 0.06 & 4406.98 \textpm 53.11 & 2146.67 \textpm 66.98 \\
MALV & L4H4 & 32 & 1 & 0.26 \textpm 0.05 & 0.98 \textpm 0.06 & 1.62 \textpm 0.10 & 4587.65 \textpm 104.96 & 2442.67 \textpm 126.51 \\
MALV & L4H4 & 32 & 8 & 0.38 \textpm 0.01 & 1.32 \textpm 0.02 & 2.13 \textpm 0.02 & 4263.27 \textpm 73.61 & 2060.33 \textpm 54.71 \\
MALV & L6H8 & 150 & 1 & 0.28 \textpm 0.03 & 1.06 \textpm 0.02 & 1.74 \textpm 0.02 & 4568.92 \textpm 53.91 & 2406.00 \textpm 36.36 \\
MALV & L6H8 & 150 & 8 & 0.37 \textpm 0.04 & 1.25 \textpm 0.06 & 2.11 \textpm 0.16 & 4410.64 \textpm 86.15 & 2165.33 \textpm 97.74 \\
MALV & L6H8 & 32 & 1 & 0.25 \textpm 0.02 & 0.95 \textpm 0.04 & 1.68 \textpm 0.04 & 4624.45 \textpm 50.37 & 2464.33 \textpm 54.92 \\
MALV & L6H8 & 32 & 8 & 0.33 \textpm 0.01 & 1.21 \textpm 0.02 & 2.05 \textpm 0.04 & 4282.22 \textpm 26.94 & 2059.00 \textpm 40.42 \\
M & L4H4 & 150 & 1 & 0.23 \textpm 0.01 & 0.83 \textpm 0.01 & 1.41 \textpm 0.02 & 5259.43 \textpm 44.34 & 3020.33 \textpm 8.50 \\
M & L4H4 & 150 & 8 & 0.27 \textpm 0.02 & 0.95 \textpm 0.08 & 1.52 \textpm 0.09 & 5192.75 \textpm 48.75 & 2869.00 \textpm 47.55 \\
M & L4H4 & 32 & 1 & 0.23 \textpm 0.02 & 0.99 \textpm 0.03 & 1.62 \textpm 0.07 & 4919.37 \textpm 41.15 & 2738.33 \textpm 52.22 \\
M & L4H4 & 32 & 8 & 0.27 \textpm 0.02 & 1.01 \textpm 0.04 & 1.63 \textpm 0.04 & 4856.83 \textpm 51.39 & 2607.67 \textpm 62.53 \\
M & L6H8 & 150 & 1 & 0.23 \textpm 0.03 & 0.83 \textpm 0.05 & 1.37 \textpm 0.06 & 5295.42 \textpm 109.32 & 3053.67 \textpm 124.08 \\
M & L6H8 & 150 & 8 & 0.24 \textpm 0.01 & 0.90 \textpm 0.02 & 1.55 \textpm 0.02 & 5302.24 \textpm 69.54 & 2979.33 \textpm 87.45 \\
M & L6H8 & 32 & 1 & 0.21 \textpm 0.02 & 0.88 \textpm 0.07 & 1.50 \textpm 0.07 & 4869.63 \textpm 15.27 & 2713.67 \textpm 22.87 \\
M & L6H8 & 32 & 8 & 0.27 \textpm 0.02 & 1.04 \textpm 0.02 & 1.71 \textpm 0.04 & 4836.99 \textpm 46.22 & 2583.67 \textpm 20.04 \\


==> tables/vines_arch_epe_gpu.tex <==
MALVYMTSK & L4H4 & 150 & 1 & 32.51 \textpm 0.25 & 62.17 \textpm 0.23 & 73.78 \textpm 0.42 & 16.84 \textpm 0.09 & 3.00 \textpm 0.00 \\
MALVYMTSK & L4H4 & 150 & 8 & 38.71 \textpm 0.02 & 68.97 \textpm 0.55 & 79.65 \textpm 0.17 & 13.80 \textpm 0.07 & 2.00 \textpm 0.00 \\
MALVYMTSK & L4H4 & 32 & 1 & 26.23 \textpm 0.67 & 55.80 \textpm 0.58 & 68.97 \textpm 0.65 & 20.07 \textpm 0.31 & 4.00 \textpm 0.00 \\
MALVYMTSK & L4H4 & 32 & 8 & 34.54 \textpm 0.52 & 65.02 \textpm 0.37 & 76.01 \textpm 0.34 & 15.20 \textpm 0.25 & 3.00 \textpm 0.00 \\
MALVYMTSK & L6H8 & 150 & 1 & 31.28 \textpm 0.21 & 61.62 \textpm 0.16 & 73.65 \textpm 0.41 & 17.32 \textpm 0.17 & 3.00 \textpm 0.00 \\
MALVYMTSK & L6H8 & 150 & 8 & 39.02 \textpm 0.56 & 69.57 \textpm 0.48 & 79.44 \textpm 0.27 & 13.67 \textpm 0.32 & 2.00 \textpm 0.00 \\
MALVYMTSK & L6H8 & 32 & 1 & 26.28 \textpm 1.12 & 55.10 \textpm 0.37 & 67.98 \textpm 0.52 & 20.29 \textpm 0.22 & 4.00 \textpm 0.00 \\
MALVYMTSK & L6H8 & 32 & 8 & 34.64 \textpm 0.31 & 64.76 \textpm 0.64 & 76.17 \textpm 0.60 & 15.22 \textpm 0.44 & 3.00 \textpm 0.00 \\
MALVYMT & L4H4 & 150 & 1 & 33.06 \textpm 0.60 & 64.03 \textpm 0.28 & 75.63 \textpm 0.53 & 15.88 \textpm 0.33 & 3.00 \textpm 0.00 \\
MALVYMT & L4H4 & 150 & 8 & 38.88 \textpm 0.34 & 68.89 \textpm 0.18 & 79.13 \textpm 0.33 & 14.19 \textpm 0.12 & 2.00 \textpm 0.00 \\
MALVYMT & L4H4 & 32 & 1 & 27.64 \textpm 0.25 & 57.96 \textpm 0.51 & 70.72 \textpm 0.34 & 18.97 \textpm 0.15 & 4.00 \textpm 0.00 \\
MALVYMT & L4H4 & 32 & 8 & 35.37 \textpm 0.75 & 66.54 \textpm 0.28 & 77.58 \textpm 0.48 & 14.69 \textpm 0.21 & 3.00 \textpm 0.00 \\
MALVYMT & L6H8 & 150 & 1 & 33.15 \textpm 0.89 & 63.84 \textpm 0.32 & 75.05 \textpm 0.41 & 16.49 \textpm 0.60 & 3.00 \textpm 0.00 \\
MALVYMT & L6H8 & 150 & 8 & 38.79 \textpm 0.15 & 69.03 \textpm 0.33 & 79.57 \textpm 0.10 & 14.16 \textpm 0.35 & 2.00 \textpm 0.00 \\
MALVYMT & L6H8 & 32 & 1 & 27.21 \textpm 0.15 & 57.53 \textpm 0.23 & 70.52 \textpm 0.10 & 19.05 \textpm 0.23 & 4.00 \textpm 0.00 \\
MALVYMT & L6H8 & 32 & 8 & 35.85 \textpm 0.34 & 66.44 \textpm 0.75 & 77.42 \textpm 0.54 & 14.38 \textpm 0.50 & 3.00 \textpm 0.00 \\
MALV & L4H4 & 150 & 1 & 28.95 \textpm 0.37 & 59.36 \textpm 0.34 & 71.30 \textpm 0.26 & 19.09 \textpm 0.09 & 3.67 \textpm 0.47 \\
MALV & L4H4 & 150 & 8 & 34.53 \textpm 0.33 & 64.62 \textpm 0.55 & 75.77 \textpm 0.27 & 16.23 \textpm 0.47 & 3.00 \textpm 0.00 \\
MALV & L4H4 & 32 & 1 & 24.10 \textpm 0.41 & 52.42 \textpm 0.29 & 65.69 \textpm 0.15 & 23.83 \textpm 0.56 & 5.00 \textpm 0.00 \\
MALV & L4H4 & 32 & 8 & 30.85 \textpm 0.71 & 62.04 \textpm 0.77 & 74.37 \textpm 0.51 & 16.81 \textpm 0.42 & 3.00 \textpm 0.00 \\
MALV & L6H8 & 150 & 1 & 28.37 \textpm 0.27 & 58.63 \textpm 0.09 & 71.13 \textpm 0.17 & 19.17 \textpm 0.52 & 4.00 \textpm 0.00 \\
MALV & L6H8 & 150 & 8 & 34.42 \textpm 0.76 & 64.96 \textpm 0.75 & 76.30 \textpm 0.37 & 16.32 \textpm 0.12 & 3.00 \textpm 0.00 \\
MALV & L6H8 & 32 & 1 & 24.20 \textpm 0.27 & 51.56 \textpm 0.34 & 65.54 \textpm 0.26 & 23.78 \textpm 0.10 & 5.00 \textpm 0.00 \\
MALV & L6H8 & 32 & 8 & 31.52 \textpm 0.19 & 61.71 \textpm 0.16 & 74.67 \textpm 0.39 & 16.84 \textpm 0.22 & 3.00 \textpm 0.00 \\
M & L4H4 & 150 & 1 & 17.55 \textpm 0.69 & 42.43 \textpm 0.51 & 55.10 \textpm 0.54 & 40.09 \textpm 1.01 & 8.00 \textpm 0.00 \\
M & L4H4 & 150 & 8 & 17.96 \textpm 0.23 & 41.78 \textpm 0.32 & 53.65 \textpm 0.33 & 47.35 \textpm 0.36 & 8.67 \textpm 0.47 \\
M & L4H4 & 32 & 1 & 18.55 \textpm 0.28 & 44.17 \textpm 0.90 & 57.62 \textpm 0.95 & 34.09 \textpm 0.25 & 7.33 \textpm 0.47 \\
M & L4H4 & 32 & 8 & 19.42 \textpm 0.26 & 46.40 \textpm 0.63 & 58.80 \textpm 0.17 & 34.84 \textpm 0.93 & 7.00 \textpm 0.00 \\
M & L6H8 & 150 & 1 & 16.59 \textpm 0.74 & 41.57 \textpm 0.47 & 54.58 \textpm 0.51 & 40.50 \textpm 1.65 & 8.33 \textpm 0.47 \\
M & L6H8 & 150 & 8 & 17.37 \textpm 0.45 & 41.20 \textpm 0.19 & 53.30 \textpm 0.28 & 47.26 \textpm 0.77 & 9.00 \textpm 0.00 \\
M & L6H8 & 32 & 1 & 17.90 \textpm 0.29 & 43.17 \textpm 0.65 & 56.22 \textpm 0.27 & 34.21 \textpm 0.25 & 8.00 \textpm 0.00 \\
M & L6H8 & 32 & 8 & 19.69 \textpm 0.58 & 45.47 \textpm 0.32 & 58.01 \textpm 0.61 & 35.24 \textpm 0.32 & 7.00 \textpm 0.00 \\


==> tables/yc2_arch_epe_gpu.tex <==
MALVYMTSK & L4H4 & 150 & 1 & 5.74 \textpm 0.50 & 20.63 \textpm 1.03 & 28.24 \textpm 0.46 & 65.94 \textpm 2.30 & 31.67 \textpm 1.70 \\
MALVYMTSK & L4H4 & 150 & 8 & 8.66 \textpm 1.00 & 28.48 \textpm 0.41 & 39.97 \textpm 1.13 & 41.65 \textpm 1.22 & 16.00 \textpm 0.00 \\
MALVYMTSK & L4H4 & 32 & 1 & 2.27 \textpm 0.30 & 10.11 \textpm 0.30 & 17.48 \textpm 0.86 & 96.47 \textpm 2.20 & 61.33 \textpm 1.89 \\
MALVYMTSK & L4H4 & 32 & 8 & 7.77 \textpm 0.71 & 19.90 \textpm 0.71 & 29.94 \textpm 0.80 & 61.37 \textpm 0.83 & 29.00 \textpm 1.41 \\
MALVYMTSK & L6H8 & 150 & 1 & 6.15 \textpm 0.98 & 18.12 \textpm 1.13 & 29.21 \textpm 1.26 & 65.17 \textpm 1.69 & 30.00 \textpm 2.16 \\
MALVYMTSK & L6H8 & 150 & 8 & 9.55 \textpm 0.30 & 30.50 \textpm 0.80 & 43.45 \textpm 1.69 & 39.84 \textpm 1.08 & 14.33 \textpm 1.25 \\
MALVYMTSK & L6H8 & 32 & 1 & 2.99 \textpm 0.30 & 10.28 \textpm 0.89 & 16.99 \textpm 0.40 & 92.55 \textpm 2.09 & 60.00 \textpm 1.41 \\
MALVYMTSK & L6H8 & 32 & 8 & 6.72 \textpm 0.41 & 19.82 \textpm 0.80 & 30.50 \textpm 0.30 & 60.79 \textpm 1.20 & 29.33 \textpm 1.25 \\
MALVYMT & L4H4 & 150 & 1 & 6.55 \textpm 1.50 & 20.47 \textpm 2.38 & 29.85 \textpm 1.21 & 57.63 \textpm 0.83 & 28.00 \textpm 0.82 \\
MALVYMT & L4H4 & 150 & 8 & 10.52 \textpm 1.00 & 29.77 \textpm 1.02 & 40.53 \textpm 1.05 & 40.29 \textpm 0.49 & 16.67 \textpm 0.47 \\
MALVYMT & L4H4 & 32 & 1 & 2.75 \textpm 0.41 & 12.78 \textpm 0.30 & 19.17 \textpm 1.21 & 86.37 \textpm 3.46 & 53.33 \textpm 2.05 \\
MALVYMT & L4H4 & 32 & 8 & 7.36 \textpm 0.98 & 21.93 \textpm 2.00 & 33.01 \textpm 0.40 & 53.62 \textpm 0.37 & 25.00 \textpm 0.82 \\
MALVYMT & L6H8 & 150 & 1 & 6.47 \textpm 0.70 & 19.98 \textpm 0.89 & 31.47 \textpm 0.80 & 56.81 \textpm 0.17 & 26.67 \textpm 1.70 \\
MALVYMT & L6H8 & 150 & 8 & 9.06 \textpm 0.30 & 28.96 \textpm 0.75 & 42.23 \textpm 0.52 & 39.32 \textpm 1.00 & 15.33 \textpm 0.47 \\
MALVYMT & L6H8 & 32 & 1 & 2.91 \textpm 1.10 & 11.33 \textpm 0.80 & 17.88 \textpm 0.50 & 92.77 \textpm 1.22 & 57.33 \textpm 1.70 \\
MALVYMT & L6H8 & 32 & 8 & 7.12 \textpm 0.50 & 21.60 \textpm 1.30 & 32.69 \textpm 0.30 & 54.19 \textpm 1.26 & 24.00 \textpm 0.82 \\
MALV & L4H4 & 150 & 1 & 2.75 \textpm 0.64 & 10.11 \textpm 1.21 & 16.42 \textpm 1.49 & 104.00 \textpm 3.32 & 71.67 \textpm 4.64 \\
MALV & L4H4 & 150 & 8 & 2.91 \textpm 0.20 & 11.00 \textpm 1.32 & 18.28 \textpm 0.50 & 90.72 \textpm 1.41 & 56.33 \textpm 2.49 \\
MALV & L4H4 & 32 & 1 & 1.86 \textpm 0.30 & 8.01 \textpm 0.34 & 12.54 \textpm 0.61 & 110.85 \textpm 2.99 & 77.00 \textpm 5.35 \\
MALV & L4H4 & 32 & 8 & 3.72 \textpm 0.30 & 11.73 \textpm 1.14 & 17.88 \textpm 0.46 & 91.36 \textpm 2.13 & 61.00 \textpm 2.16 \\
MALV & L6H8 & 150 & 1 & 2.59 \textpm 0.30 & 10.28 \textpm 0.80 & 15.37 \textpm 0.94 & 104.97 \textpm 0.85 & 74.33 \textpm 1.25 \\
MALV & L6H8 & 150 & 8 & 3.72 \textpm 0.30 & 11.08 \textpm 0.30 & 17.72 \textpm 0.40 & 90.04 \textpm 2.47 & 58.00 \textpm 4.55 \\
MALV & L6H8 & 32 & 1 & 1.78 \textpm 0.83 & 7.52 \textpm 0.91 & 13.19 \textpm 0.64 & 108.75 \textpm 2.00 & 79.33 \textpm 2.49 \\
MALV & L6H8 & 32 & 8 & 2.51 \textpm 0.30 & 11.97 \textpm 1.09 & 16.99 \textpm 2.07 & 94.69 \textpm 3.27 & 63.33 \textpm 2.36 \\
M & L4H4 & 150 & 1 & 2.75 \textpm 1.02 & 9.87 \textpm 1.16 & 15.37 \textpm 1.09 & 104.01 \textpm 2.62 & 71.33 \textpm 4.03 \\
M & L4H4 & 150 & 8 & 2.99 \textpm 0.50 & 10.68 \textpm 1.21 & 18.12 \textpm 0.41 & 98.06 \textpm 2.63 & 64.67 \textpm 3.09 \\
M & L4H4 & 32 & 1 & 1.94 \textpm 0.20 & 9.39 \textpm 0.50 & 15.70 \textpm 0.11 & 102.82 \textpm 2.98 & 71.67 \textpm 3.30 \\
M & L4H4 & 32 & 8 & 3.48 \textpm 0.50 & 10.84 \textpm 0.64 & 18.45 \textpm 0.34 & 95.52 \textpm 2.30 & 65.00 \textpm 0.82 \\
M & L6H8 & 150 & 1 & 2.99 \textpm 0.41 & 10.28 \textpm 1.00 & 15.70 \textpm 0.92 & 107.67 \textpm 4.27 & 74.33 \textpm 3.40 \\
M & L6H8 & 150 & 8 & 2.83 \textpm 0.46 & 11.97 \textpm 0.50 & 18.04 \textpm 0.30 & 96.83 \textpm 0.79 & 60.33 \textpm 2.05 \\
M & L6H8 & 32 & 1 & 2.51 \textpm 0.41 & 8.41 \textpm 0.50 & 14.40 \textpm 1.02 & 107.28 \textpm 1.57 & 77.00 \textpm 6.48 \\
M & L6H8 & 32 & 8 & 2.18 \textpm 0.71 & 10.19 \textpm 0.52 & 18.45 \textpm 0.52 & 91.67 \textpm 2.00 & 59.33 \textpm 1.70 \\

